A Convolutional Transformation Network for Malware Classification

Modern malware evolves various detection avoidance techniques to bypass the state-of-the-art detection methods. An emerging trend to deal with this issue is the combination of image transformation and machine learning techniques to classify and detect malware. However, existing works in this field only perform simple image transformation methods that limit the accuracy of the detection. In this paper, we introduce a novel approach to classify malware by using a deep network on images transformed from binary samples. In particular, we first develop a novel hybrid image transformation method to convert binaries into color images that convey the binary semantics. The images are trained by a deep convolutional neural network that later classifies the test inputs into benign or malicious categories. Through the extensive experiments, our proposed method surpasses all baselines and achieves 99.14% in terms of accuracy on the testing set.

==> parts/intro-backup.tex <==
The number of new malware and variants on the Internet has been continuously increasing with the help of various automated toolkits, which employ different techniques such as encryption, obfuscation, packing to evade the detection of anti-malware scanners~\cite{MalDet:Surveys:2017,evading:2017}.  %The total number of new malware variants added in 2013 and 2014 were 252 million and 317 million (a 26\% increase from 2013), respectively (Symantec, 2015 \cite{symantec2015}). 
When developing malware, the authors employ obfuscation techniques to create a new variant of an existing malware. The new variant can do the same functionality as the old one but its look is different. To detect such malware, we need to capture similarities between malware variants, and benign applications. Rather than relying on a unique signature for a particular malware, describe the malware by its characteristics and behaviors. Static features such as \textit{strings} or \textit{imports} \cite{schultz2001data} can help to get the overview of malware . However, static analysis has its own limitation \cite{moser2007limits} as they can be obfuscated easily. The static analysis looks at instructions \cite{christodorescu2005semantics} disassembly code of malware and learn its behavior from various representation such as function call graph \cite{hu2009large}.  
Dynamic analysis requires executing an executable in an isolated environment \cite{willems2007toward} , \cite{rieck2008learning} get API calls \cite{bose2008behavioral}, \cite{bayer2006dynamic}, system changes \cite{bailey2007automated}, they can give more details on what malware really does. However, it is a time-consuming process and only examines a single execution path. They also suffer from several anti-analysis techniques such as anti-debugging, virtual machine. In addition, to run a program, we have to know about the information about its type which limits analysis capability. 
 

Each analysis has an advantages and disadvantages depending on the amount of information we are going to extract. At binary level, we can do extract non overlapping byte sequences \cite{schultz2001data} or n-gram \cite{kolter2006learning}, by considering a program as a stream of bytes regardless of its type. Binary is,just 0 or 1, the lowest level where th  . Our approach works on this level as it is resilient to anti analysis techniques. However, the main challenge is that byte value gives very little semantic information about malware. We tackle this problem by adding and highlighting important sequences visually using entropy technique. A binary is transformed into a color image where its channels encodes semantic information. By visualizing continuous sequences of same semantic entropy values, the image can highlight important sections in binary for further analysis such as packed or encrypted sections or keys, passwords which meant to be hidden from human view.  To select the best color scheme to represent semantic meaning of the binary data. Our search begins a simple color scheme where bytes are classified into a small number of categories to get the overview of the structures of file. Then, we takes the byte stream and split them into blocks of 32 bit and calculate the Shanon entropy on them. With the second scheme, we can locate encrypted or packed sections. 
From 256 different byte values, we compress that down into a few common character class , calculate byte entropy over sliding window ,  Each of these color scheme is useful for analyzing malware. The character class scheme covers the most common padding bytes, nicely highlights strings in malware. The entropy scheme lets you quickly pick out encrypted and compressed sections. 

To automatically recognize malware variants, their shared patterns should be learned. Based on the observation that image representations of different from the same family appear to be similar. As if malware authors make a small change in the original binary, its image retain the global structure. We built a deep neural network to learn the global patterns shared among malware. Each layer in the network learn 
Our proposed method consists of the following steps in a supervised training phase. First, given an executable (benign or malicious), we divide its into blocks of sequence and calculate the Shanon entropy value for each block. Next, these blocks are analyzed conditionally and assigned to corresponding color. The transformed images are fed into a few Convolutional neural network (CNN) layers which pick out in variant features. Finally, the output of the last CNN layer is input into the fully connected layer to output the decision on the input file. In order to support understanding image features, we wrote a python script to visualize learned features.   
% The reason behind that large number of variants is that 
% Malware authors reuse some modules or change small parts of the original source code to produce a new variant. To fight the ever-increasing proliferation of novel malware, antivirus (AV) vendors have turned to emulation-based automated dynamic malware analysis instead of using certain character strings or patterns, i.e., signatures to detect malware variants (Christodorescu \textit{et al.} \cite{christodorescu2004testing}).   
% \phu{this is quite old}. 
% Malware authors have responded by creating malware that attempts to evade detection by behaving benignly while running in an emulator \phu{More details and references are better here}. They use the techniques of polymorphism and metamorphism to change the form of each instance malware in order to evade "pattern-matching" during the detection and investigative process. To efficiently and effectively the enormous amount of malicious variant, it has been proposed that by comparing the similarity of malware instance to  determine whether submitted samples are merely variations of existing ones. And static analysis of polymorphic 
% \phu{this terminology needs to be explained} 
% malware which changes  plays an important role. It describes the process of analyzing the code or structure of a program to determine its function. The similarities of these variants can be computed by using control flow graph but it suffers from code obfuscation. Full binary fuzzing hashing of malware does not perform well in many cases such as packing, reordering of functions, and partial code reuse \cite{raygoza2009automated}. Analyzing raw binaries and extract byte-streams does not give much information because it does not contain semantic of malware behaviors.
% \phu{Explanation!}. 
% Executing the malware in a virtual environment, capture its execution trace and then similarity of its behavior~\cite{park2010fast,shaid2014malware} is complex and time consuming. 
% The binaries are divided into different sections which can be easily seen when viewed as an image. 
% Images can capture small changes yet retain the global structure. This paper is highly motivated by the work which based on the observation that images of different malware variants from the same family appear to be very similar. These images belong to a different family are distinct. Specifically, if old malware is re-used to create new malware binaries, the resulting ones would be having common structures that were present in the original binaries. 
% Our approach is not only subject to anti-tracing, anti reverse engineering logic, or many common code obfuscation strategies now incorporated into packed binaries, but also capable with malware which has sections that are packed - encrypted or obfuscated. In our images, large areas of very high entropy are usually packed or encrypted sections, smaller areas might be keys, passwords, or other chunks of data meant to be hidden from view.
% Our goal is not to simply state that two samples are similar, but also help analysts to identify which of their components make them similar.   
% Because of automated tools, similar modules may appear in malware variants, and these similar modules can be used to detect variants. Structure layout 
% Most of antivirus programs use certain character strings or patterns, i.e., signatures to detect malware~\cite{christodorescu2004testing}. However, signature-based detection methods can be avoided if diverse detection avoidance techniques are used in malware \cite{moser2007limits}. Thus, malware researchers have studied various analysis techniques to respond to malware variants and detection avoidance techniques. To address the problem of analysis of malware binary objects, we present binary transformation techniques that map a binary file to a color image. 

% This paper is highly motivated by the work in which is based on the observation that images of different malware samples from the same family appear to be similar while images of malware samples belong to a different family are distinct. 
% Moreover, if old malware is re-used to create new malware binaries the resulting ones would be very similar visually. In addition, as malware authors only change a small part of the code to produce new variants, images are useful to detect small changes while retain the global structure. In consequence, malware variants belonging to the same family appear to be very similar as images while also being distinct from images of other families.  

% Visualizing malware at binary-level ({Nataraj \textit{et al.}~\cite{nataraj2011malware}) provides a quick view of the overall structure of the file which is useful for analytic tasks. 
% It gives more information about the structure of the malware. The entire structural layout can also easily be seen. 
% Instead of converting malware binary into images based on binary values, we are looking at a variety of semantic meaning of the binary data. First, we begin by picking a color scheme. From 256 different byte values, we compress that down into a few common character class (described in Section []), calculate byte entropy over sliding window (Section [?]),  Each of these color scheme is useful for analyzing malware. The character class scheme covers the most common padding bytes, nicely highlights strings in malware. The entropy scheme lets you quickly pick out encrypted and compressed sections. 

%\tam{TRY TO ADD MORE RELATED WORKS HERE: JUST BRIEF INFORMATION, DON'T NEED DETAILS HERE.}

%\phu{Agree! Focus on several closest works with their limitations and motivate our work (why our work is important).}

% In order to protect legitimate users from the attacks, the majority of anti-malware software products (e.g., Comodo, Symantec, Kaspersky) use the signature-based method of detection \cite{ye2017survey}. Signature is a short string of bytes, which is unique for each known malware so that its future examples can be correctly classified with a small error rate. However, this method can be easily evaded by obfuscation techniques \cite{you2010malware}
% In order to deal with huge volume of malware, it is necessary to develop
% systems that are capable of automated malware analysis. Machine learning techniques, in particular machine-learning-based techniques play an important role in such analysis. Machine learning for malware detection approaches include static code analysis and dynamic code analysis for extract features. Static features works by disassembling the code and exploring the control flow of the executable to look for malicious patterns such as $n$-gram from binary \cite{kolter2006learning}, string (cite). On the other hand, dynamic analysis works by executing the code in a virtual environment and a behavioral report characterizing the executable is generated based on the execution trace. Both these techniques have their pros and cons. 

%\kha{ 
% Another approach transfers malware into a common image for classification. The initial approach begin \cite{nataraj2011malware},  \cite{liu2016malware} 
%}

% * <vuducly151092@gmail.com> 2017-08-01T01:14:19.668Z:
%
% ^.
% * <vuducly151092@gmail.com> 2017-08-01T01:13:04.022Z:
% 
% I've added some reference papers related to our work. 
% 
% ^ <vuducly151092@gmail.com> 2017-08-01T01:14:04.490Z.

% Kolter et al \cite{kolter2004learning} used n-gram (instead of non-overlapping byte sequences) and a data mining method to detect malicious executables. They used different classifiers including Naive-Bayes, Support Vector Machine, Decision Tree and their boosted versions. 
% * <phunghuuphu@gmail.com> 2017-08-01T13:54:42.229Z:
% 
% I think in this section, we just need to give a brief overview of the literature and highlight what problems have not been solved so that our work will fill the gap
% 
% ^.

% Dahl et al. \cite{dahl2013large} tried to classify malware on a large scale using random projections and neural networks. However, they did not report on the advantages of increasing the number of neural network layers.

% Saxe et al. \cite{saxe2015deep} used feed-forward neural networks to classify malware. They used static features such as PE import features or metadata features which are easily obfuscated. Additionally, it usually takes time to extract and build these features.

% Huang et al. \cite{huang2016mtnet}, on the other hand, used up to four hidden layers of a feed-forward neural network  on evaluating multi-task learning ideas. However, they needed to extract arguments from the API calls as well as API name trigrams. Additionally, to reduce the input space, they had to use feature selection which increased the preprocessing overhead.

% Pascanu et al. \cite{pascanu2015malware} used recurrent neural networks for modeling system call sequences. In order to construct a `language model' for malware, they tested LSTM and GRU, and reported good classification performance. However, they did not test deep learning approaches.

% Liu and Bao \cite{liu2016malware} convert disassembly files into gray-scale images. In order to improve the efficiency, we use the local mean method to compress gray-scale images, which are mapped into feature vectors. To classify malware, we propose a novel ensemble learning which is based on K-means and the diversity selection.

% \cite{nataraj2011malware} propose a simple yet effective method for visualizing and classifying malware using image processing techniques. Malware binaries are visualized as gray-scale images, with the observation that for many malware families, the images belonging to the same family appear very similar in layout and texture.
% In their work, they computed image based features to characterize malware . For that purpose, to compute texture features they used GIST 

% \cite{annachhatre2015hidden} train multiple hidden Markov model  on a variety of compilers and malware generators. More than 8,000 malware samples are then scored against these models and separated into clusters based on the resulting scores. We observe that the clustering results could be used to classify the malware samples into their appropriate families with good accuracy.
% The main benefit of visualizing malware as an image is that the different sections of a binary can be easily differentiated.  

% \cite{shaid2014malware} showcase a new technique for malware
% visualization that will highlight the behavioral aspects of
% malware. The technique will display malware behavior in the
% form of images (called behavior image). The presented method
% can be used for malware analysis, detection and identification of
% malware variants.

% The 3 dimensional malware model by \cite{quist2009visualizing} on the other
% hand is a model that captures memory addresses of malware code
% execution blocks that is color coded, to represent the various state
% of the block of code, including the existence of the code on disk
% and in memory, the entropy of the code, and various other
% information that seems to be targeted towards malware
% unpacking analysis. The color coded nodes enable easy
% identification of highly compressed code, newly created code
% blocks, and other useful information which could help in the
% process of malware analysis. For example, it is trivial to find the
% Original Entry Point (OEP) of a packed executable merely by
% looking at the change in color information. 

% \cite{oliva2001modeling}


%[I JUST UPDATED THE CONTRIBUTIONS HERE.]

Our contributions are as follows:
\begin{itemize}
\item We are the first who consider binary malware samples as color images using space filling curves.
\item Second, we explore different methods to convert the malware samples into images. Instead of converting malware binary into images based on binary values, we are looking at the level of the semantic meaning of the binary data, for example, low, ascii, and high values.  
\item Last but not least, we also investigate the usage of learned features in deep learning for classifying malware samples. Through extensive experiments, our proposed method achieves 98.82\% of accuracy on the test set. 

\end{itemize}

The composition of this paper is as follows: Section~\ref{sec:related} describes related work on malware analysis, detection, and classification methods. In Section ~\ref{sec:method}, a malware analysis using color images is proposed, and experimental results are shown in Section~\ref{sec:experiments}. %In Section [?], limitations and future work are discussed. 
Finally, in Section~\ref{sec:conc}, the conclusions of this paper are presented  future work are discussed. 

==> parts/relatedwork-old.tex <==
\subsection{Malware classification}
\paragraph{API monitoring} Rieck \textit{et al.}~\cite{rieck2008learning}  feature set includes operations on system resources, for example creating a service for persistence purpose. The feature vectors are then learned by Support vector machine classifier.
\paragraph{Byte sequence} Kolter \textit{et al.}~\cite{kolter2004learning} use overlapping byte sequences or n-grams as features.
\paragraph{File header}: Dahl \textit{et al.} \cite{dahl2013large}, Saxe \textit{et al.}~\cite{saxe2015deep} extracted static PE import features or metadata features and used random projections and neural networks to classify malware.
% \subsection{Background}
% In this section, we first review the progress of image classification. Then, we summarize the malware classification and the integration of the image transformation into the malware classification.  


% \subsection{Image classification}

% Image classification is a fundamental problem in computer vision. In the early stage, Haralick \textit{et al.} \cite{haralick1973textural} describes some easily computable textural features based on graytone spatial dependancies, and illustrates their application in category-identification tasks. Later, LeCun \textit{et al.} \cite{lecun1998gradient} proposed Convolutional neural networks (ConvNets or CNNs) by stacking several convolutional operators into a network. CNNs can create a hierarchy of progressively more abstract features and show a good performance on hand-writing digit classification. However, the limitation of  hardware resource restricted CNNs from further investigation. Therefore, there exist many works using hand-crafted features for image classification. In the global scale, GIST~\cite{oliva2001modeling} is computed over the entire image as a global image descriptor for the purposes of scene classification. In the local scale, Lowe~\cite{SIFT} introduced SIFT feature extracted from interest points. Similarly, Dalal \textit{et al.}~\cite{HOG} proposed histogram of gradients (HOG) which can be used for both image classification and object detection in a sliding window manner. 

% Recently, along with the development of GPUs, CNNs were resurrected in deep learning for image classification. Krizhevsky \textit{et al.}~\cite{krizhevsky2012imagenet} trained a large, deep convolutional neural network to classify the 1.2 million high-resolution images in the ImageNet LSVRC-2010 contest into the 1000 different classes.  The network has many layers, namely, convolution layers and max-pooling layers, and fully-connected layers with a final 1000-class softmax. Furthermore, there are many extensions to deeper networks for a higher performance in terms of classification rate~\cite{VGG,Googlenet,ResNet}. 

% \subsection{Malware Classification }

% %\subsubsection{Meta Data based Classification}
% % Schultz \textit{et al.}~\cite{schultz2001data}, Tian \textit{et al.} ~\cite{tian2009automated}, Islam \textit{et al.} \cite{islam2013classification}, Dahl \textit{et al.} \cite{dahl2013large}, Saxe \textit{et al.}~\cite{saxe2015deep} extracted information from PE Header, hexadecimal byte sequences and strings.
% % Given a dataset: 3256 malicious and benign samples, 
% % they constructed a feature vector which represent the occurrence of DLLs, their function calls and the number of exported functions in each DLL, \textit{strings}.

% % To extract features from non PE executables, they searched for \textit{strings} in them. 
% % Schultz \textit{et al.} and Kolter \textit{et al.}~\cite{kolter2004learning} extracted overlapping and non overlapping byte sequences, respectively from binaries and built classifiers to differentiate benign and malicious byte sequences.   
% % The last feature set contains byte sequences taken by hexademcimal representaion of binary files. Similarly each byte sequence is a binary feature. The authors claimed that there were a difference between benign and malicious class at bytecode level. DLLs, strings and byte sequence features were then fed into the Ripper (Cohen and William ~\cite{cohen1995fast}) and Naive Bayes. Their features such as Strings and other PE header information are easily obfuscated by packing tools however.  

% % In ~\cite{kolter2004learning} Kolter \textit{et al.} extracted byte n-grams as features. Because of large number of n-grams, they then selected the most significant ones using their information gain. Specifically, processing 1651 malware and 1971 goodware resulted in 255 million n-grams. They are then reduced to 500 features. They trained the features using Naive Bayes, J48, SVM, IBk and their boost version and achieved the area under curve of 0.996. The number of features are proportional to the size of dataset which increases computing overhead. 
% % Additionally, n-gram features are not easy to understand to human  

% % Static based features suffer from binary obfuscation and are limited in representing true behavior of malware. In \cite{rieck2008learning}, Rieck \textit{et al.} adopted the dynamic approach to classify malware families. The program is executed in a sandbox and its behavior is collected. The behavior feature set includes operations on system resources, for example creating a service for persistence purpose. The feature vectors are then learned by Support vector machine classifier.They evaluated their approach on two datasets of 10,072 samples of 14 families and achieved 88\% of accuracy in average. This approach is however suffer from malware evasion techniques. 
% % Kong \textit{et al.} ~\cite{kong2013discriminant} built a function call graph on disassembly code and measure similarity of graphs of malware and clean programs. 
% % Siddiqui \textit{et al.} ~\cite{siddiqui2009detecting}, Tian \textit{et al. } ~\cite{tian2008function}, ~\cite{islam2013classification} used function length as features, however it is easy to modify the length of function by using obfuscation techniques such as dead code injection. 

% % Dive into assembly code in a function, Bilar and Daniel ~\cite{bilar2007opcodes} counted frequency of opcodes in malicious and benign program dataset. After analyzing distribution of the opcodes, they report frequent, rare opcodes in goodware and malware. The results can be used to support building detection rules based on opcodes. 

% % In ~\cite{zhang2014semantics} Zhang \textit{et al.} built the graph  representation of dependence API calls in Android bytecode. Given an application, they first locate API calls of interest, do data flow analysis to explore relationships between APIs and parameters. Then a query is made against the database of extracted graphs to find the most similar graph to the input graph. Malicious applications are then compared to the database which result in the corresponding feature vectors. These features are fed into a classifier for produce signatures for malware family identification. The classifier is tested on 2200 malware and 13500 goodware  and achieved the 5.15\% of false positive rate.

% % Shabtai \textit{et al.}~\cite{shabtai2010automated} extracted apk's properties such as size, number of zip entries. In Manifest file of an application, they extracted frequency of elements, element's name characteristics, attribute types, namespaces, unique strings and list of requested permissions. They disassemble dex files to get strings, methods, opcodes and other basic features. Then they remove irrelevant features and use feature selection algorithms to select significant features. Using the dataset of 2,850 games and applications, they achieved the accuracy of 91.8\% and the false positive of 0.172\%  

% % In ~\cite{bailey2007automated} Bailey \textit{et al.} observed 
% % Bailey \textit{et al.} adopted  proposed a method for automatically categorizing these profiles of malware into groups based on system state changes (e.g., files written, processes created). 
% % Rieck \textit{et al.} \cite{rieck2008learning}  exploit shared typical behavioral patterns for classification of malware and propose a method for learning and discrimination of malware behavior. 

% % Dahl \textit{et al.} \cite{dahl2013large}, Saxe \textit{et al.}~\cite{saxe2015deep} extracted static PE import features or metadata features and used random projections and neural networks to classify malware. However, they did not report on the advantages of increasing the number of neural network layers. Huang \textit{et al.}~\cite{huang2016mtnet}, on the other hand, used up to four hidden layers of a feed-forward neural network  on evaluating multi-task learning ideas. However, they needed to extract arguments from the API calls as well as API name trigrams. Additionally, to reduce the input space, they had to use feature selection which increased the preprocessing overhead.

% \subsubsection{Image-based Malware Classification}

% % There exist several methods converting binary files into color images in order to cast the malware classification to the image classification problem. 
% % Two observations behind the use of representing an binary in image form are that it can capture semantic features of the binary and will not suffer from anti dynamic analyses introduced by malware. 

% (Zhang \textit{et al.} \cite{zhang2014semantics}) proved the former hypothesis by introducing API call dependency graphs. Then these graphs are processed by a graph similarity algorithm to output feature vectors They however put a lot of effort on finding the entry point, data flow analysis.

% Our work is most closely related to that of Nataraj (Nataraj \textit{et al.}. \cite{nataraj2011malware}) proposed a simple yet effective method for visualizing and classifying malware on gray-scale images by exploiting their layout and texture. However, we instead transform binaries into color images with hilbert curves.  

% % (Annachhatre \textit{et al.} \cite{annachhatre2015hidden}) trained multiple hidden Markov model  on a variety of compilers and malware generators. More than 8,000 malware samples are then scored against these models and separated into clusters based on the resulting scores. We observe that the clustering results could be used to classify the malware samples into their appropriate families with good accuracy. The main benefit of visualizing malware as an image is that the different sections of a binary can be easily differentiated.  

% Shaid \textit{et al.}~\cite{shaid2014malware} execute samples and represent their behavior in the form of images.(Quist \textit{et al.} \cite{quist2009visualizing}) on the other hand  captures memory addresses of malware code execution blocks to represent the existence of the code on disk and in memory, the entropy of the code. 
% % The color coded nodes enable easy
% % identification of highly compressed code, newly created code
% % blocks, and other useful information which could help in the
% % process of malware analysis. For example, it is trivial to find the Original Entry Point (OEP) of a packed executable merely by looking at the change in color information. 

% % (Hu \textit{et al.} \cite{hu2009large}) design, implement and evaluate a malware database management system called SMIT (Symantec Malware Indexing Tree) that can efficiently make such determination based on malware's function-call graphs. 



% %  propose a simple yet effective method for visualizing and classifying malware using image processing techniques. Malware binaries are visualized as gray-scale images, with the observation that for many malware families, the images belonging to the same family appear very similar in layout and texture.

% \cite{han2015malware}  proposed a method by converting binary files into images and entropy graphs. 
% (Han \textit{et al.} \cite{han2013malware}) proposed a novel method to visually analyze malware by transforming malware binary information into image matrices.

% (Han \textit{et al.} \cite{han2014malware}) proposed method generates RGB-colored pixels on image matrices using the opcode sequences extracted from malware samples and calculates the similarities for the image matrices.

% % \phu{I think we might need to have a background section, presenting Deep Networks and Image Transformation Techniques}

% (Liu \textit{et al.} \cite{liu2016malware}) convert disassembly files into gray-scale images. In order to improve the efficiency, we use the local mean method to compress gray-scale images, which are mapped into feature vectors. To classify malware, we propose a novel ensemble learning which is based on K-means and the diversity selection.

% %\subsubsection{Feature Extraction}


% % Many people use pre-trained ConvNet models and then remove the last output layer to extract the features from ConvNets. We do not use pre-trained models. 


% % Natural images have the property of being ”‘stationary”’, meaning that the statistics of one part of the image are the same as any other part. This suggests that the features that we learn at one part of the image can also be applied to other parts of the image, and we can use the same features at all locations.

% % More precisely, having learned features over small (say 8x8) patches sampled randomly from the larger image, we can then apply this learned 8x8 feature detector anywhere in the image. Specifically, we can take the learned 8x8 features and ”‘convolve”’ them with the larger image, thus obtaining a different feature activation value at each location in the image.

% %{\color{red}Ly: I am thinking of the formalization of CNN?, we can use mathematical formula to illustrate it.}

% %{\color{red}Ly: I think that we might need to provide the background of convolutional neural network. How does it help in extracting our images?}
% % \subsubsection{GIST feature}

% % Convolution networks make use of convolution, which, in turn, exploits information contained in space (in images) or time (in sound data).
% % To learn about thousands of objects from millions of images we need a model with a large learning capacity. Our model should have lots of prior knowledge to compensate all data we do not have . Convolutional neutral network constitutes one such class of models. Their capacity can be controlled by varying their depth and breadth, and they also make strong and mostly correct assumptions about the nature of images. Thus compared to standard feed forward neutral networks with similar sized layers CNNs have much fewer connections and parameters and so they are easier to train, while theoretically best performance is likely to be only slightly worse. 
% Compared to Gist the learning network is directly fed with images rather than feature vectors thus demonstrating the ability of networks to deal with large most of low information.
% % \phu{New comment: might be we can move the related work section here. Also we need to provide citations that contemporary malware implement detection avoidance techniques}
% % Several binary analysis and text editors tools such as IDA and Hopper dissembler adapt binary visualization for easily manipulate the binary data. 

% Perdisci \textit{et al.}~\cite{perdisci2008classification}, applied pattern recognition techniques for fast detection of packed executables. Meanwhile, Lyda \textit{et al.}~\cite{lyda2007using} divided the PE file into blocks of 256 bytes. It then computes the entropy of each block, the average, and the maximum block entropy. Given a dataset of packed binaries, the authors use simple statistical inference to compute a 99.99\% confidence interval on the value of the average block entropy and maximum block entropy. Based on the lower bound of these two confidence intervals, they set two thresholds, one of the value of the the average block entropy, and one for the maximum block entropy. 

% \subsubsection{Image-based Malware Classification with Deep Learning}

%  Pascanu \textit{et al.}~\cite{pascanu2015malware} used recurrent neural networks for modeling system call sequences. In order to construct a `language model' for malware, they tested LSTM and GRU, and reported good classification performance. However, they did not test deep learning approaches.



% %\cite{oliva2001modeling}

% % \tam{TRY TO ADD MORE RELATED WORKS HERE: MORE DETAILS HERE.}
% % \phu{also, describe each related work in a couple of sentences.}

% % Several binary analysis and text editors tools such as IDA and Hopper dissembler adapt binary visualization for easily manipulate the binary data. Perdisci \textit{et al.}~\cite{perdisci2008classification}, applied pattern recognition techniques for fast detection of packed executables. Meanwhile, Lyda \textit{et al.}~\cite{lyda2007using} divided the PE file into blocks of 256 bytes. It then computes the entropy of each block, the average, and the maximum block entropy. Given a dataset of packed binaries, the authors use simple statistical inference to compute a 99.99\% confidence interval on the value of the average block entropy and maximum block entropy. Based on the lower bound of these two confidence intervals, they set two thresholds, one of the value of the the average block entropy, and one for the maximum block entropy. Liu and Bao \cite{liu2016malware} convert disassembly files into gray-scale images. In order to improve the efficiency, we use the local mean method to compress gray-scale images, which are mapped into feature vectors. To classify malware, we propose a novel ensemble learning which is based on K-means and the diversity selection.

% % There exist several methods converting binary files into color images in order to cast the malware classification to the image classification problem. \cite{nataraj2011malware} proposed a simple yet effective method for visualizing and classifying malware using image processing techniques. Malware binaries are visualized as gray-scale images, with the observation that for many malware families, the images belonging to the same family appear very similar in layout and texture.
% % In their work, they computed image based features to characterize malware . For that purpose, to compute texture features they used GIST. \cite{annachhatre2015hidden} trained multiple hidden Markov model  on a variety of compilers and malware generators. More than 8,000 malware samples are then scored against these models and separated into clusters based on the resulting scores. We observe that the clustering results could be used to classify the malware samples into their appropriate families with good accuracy. The main benefit of visualizing malware as an image is that the different sections of a binary can be easily differentiated.  Shaid \textit{et al.}~\cite{shaid2014malware} showcased a new technique for malware visualization that will highlight the behavioral aspects of malware. The technique will display malware behavior in the form of images (called behavior image). The presented method can be used for malware analysis, detection and identification of malware variants. The 3 dimensional malware model by \cite{quist2009visualizing} on the other hand is a model that captures memory addresses of malware code execution blocks that is color coded, to represent the various state of the block of code, including the existence of the code on disk and in memory, the entropy of the code, and various other information that seems to be targeted towards malware
% % unpacking analysis. The color coded nodes enable easy
% % identification of highly compressed code, newly created code
% % blocks, and other useful information which could help in the
% % process of malware analysis. For example, it is trivial to find the Original Entry Point (OEP) of a packed executable merely by looking at the change in color information. 

% % There are several efforts of using deep networks or neural networks in the classification task. Dahl \textit{et al.} \cite{dahl2013large} tried to classify malware on a large scale using random projections and neural networks. However, they did not report on the advantages of increasing the number of neural network layers. Saxe \textit{et al.}~\cite{saxe2015deep} used feed-forward neural networks to classify malware. They used static features such as PE import features or metadata features which are easily obfuscated. Additionally, it usually takes time to extract and build these features. Huang \textit{et al.}~\cite{huang2016mtnet}, on the other hand, used up to four hidden layers of a feed-forward neural network  on evaluating multi-task learning ideas. However, they needed to extract arguments from the API calls as well as API name trigrams. Additionally, to reduce the input space, they had to use feature selection which increased the preprocessing overhead. Pascanu \textit{et al.}~\cite{pascanu2015malware} used recurrent neural networks for modeling system call sequences. In order to construct a `language model' for malware, they tested LSTM and GRU, and reported good classification performance. However, they did not test deep learning approaches.



% %\cite{oliva2001modeling}

% % \tam{TRY TO ADD MORE RELATED WORKS HERE: MORE DETAILS HERE.}
% % \phu{also, describe each related work in a couple of sentences.}



\subsubsection{Meta Data based Classification}
Schultz \textit{et al.}~\cite{schultz2001data}, Tian \textit{et al.} ~\cite{tian2009automated}, Islam \textit{et al.} \cite{islam2013classification}, Dahl \textit{et al.} \cite{dahl2013large}, Saxe \textit{et al.}~\cite{saxe2015deep} extracted information from PE Header, hexadecimal byte sequences and strings.
% Given a dataset: 3256 malicious and benign samples, 
they constructed a feature vector which represent the occurrence of DLLs, their function calls and the number of exported functions in each DLL, \textit{strings}.

% To extract features from non PE executables, they searched for \textit{strings} in them. 
Schultz \textit{et al.} and Kolter \textit{et al.}~\cite{kolter2004learning} extracted overlapping and non overlapping byte sequences, respectively from binaries and built classifiers to differentiate benign and malicious byte sequences.   
% The last feature set contains byte sequences taken by hexademcimal representaion of binary files. Similarly each byte sequence is a binary feature. The authors claimed that there were a difference between benign and malicious class at bytecode level. DLLs, strings and byte sequence features were then fed into the Ripper (Cohen and William ~\cite{cohen1995fast}) and Naive Bayes. Their features such as Strings and other PE header information are easily obfuscated by packing tools however.  

% In ~\cite{kolter2004learning} Kolter \textit{et al.} extracted byte n-grams as features. Because of large number of n-grams, they then selected the most significant ones using their information gain. Specifically, processing 1651 malware and 1971 goodware resulted in 255 million n-grams. They are then reduced to 500 features. They trained the features using Naive Bayes, J48, SVM, IBk and their boost version and achieved the area under curve of 0.996. The number of features are proportional to the size of dataset which increases computing overhead. 
% Additionally, n-gram features are not easy to understand to human  

Static based features suffer from binary obfuscation and are limited in representing true behavior of malware. In \cite{rieck2008learning}, Rieck \textit{et al.} adopted the dynamic approach to classify malware families. The program is executed in a sandbox and its behavior is collected. The behavior feature set includes operations on system resources, for example creating a service for persistence purpose. The feature vectors are then learned by Support vector machine classifier.They evaluated their approach on two datasets of 10,072 samples of 14 families and achieved 88\% of accuracy in average. This approach is however suffer from malware evasion techniques. 
Kong \textit{et al.} ~\cite{kong2013discriminant} built a function call graph on disassembly code and measure similarity of graphs of malware and clean programs. 
Siddiqui \textit{et al.} ~\cite{siddiqui2009detecting}, Tian \textit{et al. } ~\cite{tian2008function}, ~\cite{islam2013classification} used function length as features, however it is easy to modify the length of function by using obfuscation techniques such as dead code injection. 

Dive into assembly code in a function, Bilar and Daniel ~\cite{bilar2007opcodes} counted frequency of opcodes in malicious and benign program dataset. After analyzing distribution of the opcodes, they report frequent, rare opcodes in goodware and malware. The results can be used to support building detection rules based on opcodes. 

% In ~\cite{zhang2014semantics} Zhang \textit{et al.} built the graph  representation of dependence API calls in Android bytecode. Given an application, they first locate API calls of interest, do data flow analysis to explore relationships between APIs and parameters. Then a query is made against the database of extracted graphs to find the most similar graph to the input graph. Malicious applications are then compared to the database which result in the corresponding feature vectors. These features are fed into a classifier for produce signatures for malware family identification. The classifier is tested on 2200 malware and 13500 goodware  and achieved the 5.15\% of false positive rate.

% Shabtai \textit{et al.}~\cite{shabtai2010automated} extracted apk's properties such as size, number of zip entries. In Manifest file of an application, they extracted frequency of elements, element's name characteristics, attribute types, namespaces, unique strings and list of requested permissions. They disassemble dex files to get strings, methods, opcodes and other basic features. Then they remove irrelevant features and use feature selection algorithms to select significant features. Using the dataset of 2,850 games and applications, they achieved the accuracy of 91.8\% and the false positive of 0.172\%  

% In ~\cite{bailey2007automated} Bailey \textit{et al.} observed 
% Bailey \textit{et al.} adopted  proposed a method for automatically categorizing these profiles of malware into groups based on system state changes (e.g., files written, processes created). 
% Rieck \textit{et al.} \cite{rieck2008learning}  exploit shared typical behavioral patterns for classification of malware and propose a method for learning and discrimination of malware behavior. 

Dahl \textit{et al.} \cite{dahl2013large}, Saxe \textit{et al.}~\cite{saxe2015deep} extracted static PE import features or metadata features and used random projections and neural networks to classify malware. However, they did not report on the advantages of increasing the number of neural network layers. Huang \textit{et al.}~\cite{huang2016mtnet}, on the other hand, used up to four hidden layers of a feed-forward neural network  on evaluating multi-task learning ideas. However, they needed to extract arguments from the API calls as well as API name trigrams. Additionally, to reduce the input space, they had to use feature selection which increased the preprocessing overhead.

\subsubsection{Image-based Malware Classification}

% There exist several methods converting binary files into color images in order to cast the malware classification to the image classification problem. 
% Two observations behind the use of representing an binary in image form are that it can capture semantic features of the binary and will not suffer from anti dynamic analyses introduced by malware. 

(Zhang \textit{et al.} \cite{zhang2014semantics}) proved the former hypothesis by introducing API call dependency graphs. Then these graphs are processed by a graph similarity algorithm to output feature vectors They however put a lot of effort on finding the entry point, data flow analysis.

Our work is most closely related to that of Nataraj (Nataraj \textit{et al.}. \cite{nataraj2011malware}) proposed a simple yet effective method for visualizing and classifying malware on gray-scale images by exploiting their layout and texture. However, we instead transform binaries into color images with hilbert curves.  

% (Annachhatre \textit{et al.} \cite{annachhatre2015hidden}) trained multiple hidden Markov model  on a variety of compilers and malware generators. More than 8,000 malware samples are then scored against these models and separated into clusters based on the resulting scores. We observe that the clustering results could be used to classify the malware samples into their appropriate families with good accuracy. The main benefit of visualizing malware as an image is that the different sections of a binary can be easily differentiated.  

Shaid \textit{et al.}~\cite{shaid2014malware} execute samples and represent their behavior in the form of images.(Quist \textit{et al.} \cite{quist2009visualizing}) on the other hand  captures memory addresses of malware code execution blocks to represent the existence of the code on disk and in memory, the entropy of the code. 
% The color coded nodes enable easy
% identification of highly compressed code, newly created code
% blocks, and other useful information which could help in the
% process of malware analysis. For example, it is trivial to find the Original Entry Point (OEP) of a packed executable merely by looking at the change in color information. 

% (Hu \textit{et al.} \cite{hu2009large}) design, implement and evaluate a malware database management system called SMIT (Symantec Malware Indexing Tree) that can efficiently make such determination based on malware's function-call graphs. 



%  propose a simple yet effective method for visualizing and classifying malware using image processing techniques. Malware binaries are visualized as gray-scale images, with the observation that for many malware families, the images belonging to the same family appear very similar in layout and texture.

\cite{han2015malware}  proposed a method by converting binary files into images and entropy graphs. 
(Han \textit{et al.} \cite{han2013malware}) proposed a novel method to visually analyze malware by transforming malware binary information into image matrices.

(Han \textit{et al.} \cite{han2014malware}) proposed method generates RGB-colored pixels on image matrices using the opcode sequences extracted from malware samples and calculates the similarities for the image matrices.

% \phu{I think we might need to have a background section, presenting Deep Networks and Image Transformation Techniques}

(Liu \textit{et al.} \cite{liu2016malware}) convert disassembly files into gray-scale images. In order to improve the efficiency, we use the local mean method to compress gray-scale images, which are mapped into feature vectors. To classify malware, we propose a novel ensemble learning which is based on K-means and the diversity selection.

%\subsubsection{Feature Extraction}


% Many people use pre-trained ConvNet models and then remove the last output layer to extract the features from ConvNets. We do not use pre-trained models. 


% Natural images have the property of being ”‘stationary”’, meaning that the statistics of one part of the image are the same as any other part. This suggests that the features that we learn at one part of the image can also be applied to other parts of the image, and we can use the same features at all locations.

% More precisely, having learned features over small (say 8x8) patches sampled randomly from the larger image, we can then apply this learned 8x8 feature detector anywhere in the image. Specifically, we can take the learned 8x8 features and ”‘convolve”’ them with the larger image, thus obtaining a different feature activation value at each location in the image.

%{\color{red}Ly: I am thinking of the formalization of CNN?, we can use mathematical formula to illustrate it.}

%{\color{red}Ly: I think that we might need to provide the background of convolutional neural network. How does it help in extracting our images?}
% \subsubsection{GIST feature}

% Convolution networks make use of convolution, which, in turn, exploits information contained in space (in images) or time (in sound data).
% To learn about thousands of objects from millions of images we need a model with a large learning capacity. Our model should have lots of prior knowledge to compensate all data we do not have . Convolutional neutral network constitutes one such class of models. Their capacity can be controlled by varying their depth and breadth, and they also make strong and mostly correct assumptions about the nature of images. Thus compared to standard feed forward neutral networks with similar sized layers CNNs have much fewer connections and parameters and so they are easier to train, while theoretically best performance is likely to be only slightly worse. 
Compared to Gist the learning network is directly fed with images rather than feature vectors thus demonstrating the ability of networks to deal with large most of low information.
% \phu{New comment: might be we can move the related work section here. Also we need to provide citations that contemporary malware implement detection avoidance techniques}
% Several binary analysis and text editors tools such as IDA and Hopper dissembler adapt binary visualization for easily manipulate the binary data. 

Perdisci \textit{et al.}~\cite{perdisci2008classification}, applied pattern recognition techniques for fast detection of packed executables. Meanwhile, Lyda \textit{et al.}~\cite{lyda2007using} divided the PE file into blocks of 256 bytes. It then computes the entropy of each block, the average, and the maximum block entropy. Given a dataset of packed binaries, the authors use simple statistical inference to compute a 99.99\% confidence interval on the value of the average block entropy and maximum block entropy. Based on the lower bound of these two confidence intervals, they set two thresholds, one of the value of the the average block entropy, and one for the maximum block entropy. 

\subsubsection{Image-based Malware Classification with Deep Learning}

 Pascanu \textit{et al.}~\cite{pascanu2015malware} used recurrent neural networks for modeling system call sequences. In order to construct a `language model' for malware, they tested LSTM and GRU, and reported good classification performance. However, they did not test deep learning approaches.



%\cite{oliva2001modeling}

% \tam{TRY TO ADD MORE RELATED WORKS HERE: MORE DETAILS HERE.}
% \phu{also, describe each related work in a couple of sentences.}

% Several binary analysis and text editors tools such as IDA and Hopper dissembler adapt binary visualization for easily manipulate the binary data. Perdisci \textit{et al.}~\cite{perdisci2008classification}, applied pattern recognition techniques for fast detection of packed executables. Meanwhile, Lyda \textit{et al.}~\cite{lyda2007using} divided the PE file into blocks of 256 bytes. It then computes the entropy of each block, the average, and the maximum block entropy. Given a dataset of packed binaries, the authors use simple statistical inference to compute a 99.99\% confidence interval on the value of the average block entropy and maximum block entropy. Based on the lower bound of these two confidence intervals, they set two thresholds, one of the value of the the average block entropy, and one for the maximum block entropy. Liu and Bao \cite{liu2016malware} convert disassembly files into gray-scale images. In order to improve the efficiency, we use the local mean method to compress gray-scale images, which are mapped into feature vectors. To classify malware, we propose a novel ensemble learning which is based on K-means and the diversity selection.

% There exist several methods converting binary files into color images in order to cast the malware classification to the image classification problem. \cite{nataraj2011malware} proposed a simple yet effective method for visualizing and classifying malware using image processing techniques. Malware binaries are visualized as gray-scale images, with the observation that for many malware families, the images belonging to the same family appear very similar in layout and texture.
% In their work, they computed image based features to characterize malware . For that purpose, to compute texture features they used GIST. \cite{annachhatre2015hidden} trained multiple hidden Markov model  on a variety of compilers and malware generators. More than 8,000 malware samples are then scored against these models and separated into clusters based on the resulting scores. We observe that the clustering results could be used to classify the malware samples into their appropriate families with good accuracy. The main benefit of visualizing malware as an image is that the different sections of a binary can be easily differentiated.  Shaid \textit{et al.}~\cite{shaid2014malware} showcased a new technique for malware visualization that will highlight the behavioral aspects of malware. The technique will display malware behavior in the form of images (called behavior image). The presented method can be used for malware analysis, detection and identification of malware variants. The 3 dimensional malware model by \cite{quist2009visualizing} on the other hand is a model that captures memory addresses of malware code execution blocks that is color coded, to represent the various state of the block of code, including the existence of the code on disk and in memory, the entropy of the code, and various other information that seems to be targeted towards malware
% unpacking analysis. The color coded nodes enable easy
% identification of highly compressed code, newly created code
% blocks, and other useful information which could help in the
% process of malware analysis. For example, it is trivial to find the Original Entry Point (OEP) of a packed executable merely by looking at the change in color information. 

% There are several efforts of using deep networks or neural networks in the classification task. Dahl \textit{et al.} \cite{dahl2013large} tried to classify malware on a large scale using random projections and neural networks. However, they did not report on the advantages of increasing the number of neural network layers. Saxe \textit{et al.}~\cite{saxe2015deep} used feed-forward neural networks to classify malware. They used static features such as PE import features or metadata features which are easily obfuscated. Additionally, it usually takes time to extract and build these features. Huang \textit{et al.}~\cite{huang2016mtnet}, on the other hand, used up to four hidden layers of a feed-forward neural network  on evaluating multi-task learning ideas. However, they needed to extract arguments from the API calls as well as API name trigrams. Additionally, to reduce the input space, they had to use feature selection which increased the preprocessing overhead. Pascanu \textit{et al.}~\cite{pascanu2015malware} used recurrent neural networks for modeling system call sequences. In order to construct a `language model' for malware, they tested LSTM and GRU, and reported good classification performance. However, they did not test deep learning approaches.



%\cite{oliva2001modeling}

% \tam{TRY TO ADD MORE RELATED WORKS HERE: MORE DETAILS HERE.}
% \phu{also, describe each related work in a couple of sentences.}

==> parts/result.tex <==
\subsection{Experimental Results}

\paragraph{Experiments on various encoding methods}
The performance of different encoding schemes is shown in Table \ref{tab:encoding_schemes}. There are two variants in each encoding: horizontal and vertical byte rendering. 

\paragraph{Experiments on using machine learning techniques on malware image}
An initial one-dimensional array, which comes before image rendering step is fed into a \emph{SVM} algorithm for classification. 
Gist features extracted from images are the inputs to kNN algorithms as \cite{nataraj2011comparative} did.
The performance of different image transformation methods and different image features are shown in Table~\ref{compare_table}. CNN performs better than GIST. Our HIT performs the best in both training set and test set. That means the HIT can be able to generalize well on unseen samples. The performance on the training set is better than the one on the validation. There is one exception that the entropy transformation performs better with new unseen data in CNN.\\ 


Regarding the GIST feature, the gray image transformation performs the best with 94\%. While using CNN features, HIT reaches the top performance with \textbf{98.82}\% accuracy. The results indicate that using color images with CNN architecture is better than grayscale images. 


\paragraph{Image understanding support} 
\begin{figure}
\centering     %%% not \center
\subfigure[Benign average]{\label{fig:a}\includegraphics[width=40mm]{figures/benign_dataset8.png}}
\subfigure[Malicious average]{\label{fig:b}\includegraphics[width=40mm]{figures/malicious_dataset8.png}}
\caption{Mean output of benign (left) and malicious (right) samples.}
\label{fig:meanviz}
\end{figure}
Fig. \ref{fig:meanviz} visualizes the output average taken from the last network in our model. We can observe that the mean outputs of benign and malicious samples are totally different. Fig. \ref{fig:a} shows that benign samples in average have almost locations in the green regions while malicious samples have more sections in the dark blue regions as shown in Fig.~\ref{fig:b}. It obviously indicates that malware are evolved with obfuscation techniques to hide visible indicators. 


% \begin{table}[!t]
% \centering
% \normalsize
% \caption{Performance comparison. The best performance of each category is highlighted with boldface font.}
% \label{tab:encoding_schemes}
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Scheme     & SVM & CNN & RNN & DNN  \\ \hline
% Vertical Gray scale &      &  &  & \\ \hline
% Horizontal Gray scale &      &  &  & \\ \hline
% Vertical Hilbert &      &  &  & \\ \hline
% Horizontal Hilbert &      &  &  & \\ \hline
% Vertical Gradient &      &  &  & \\ \hline
% Horizontal Gradient &      &  &  & \\ \hline
% Vertical Entropy &      &  &  & \\ \hline
% Horizontal Entropy &      &  &  & \\ \hline
% Vertical Class &      &  &  & \\ \hline
% Horizontal Class &      &  &  & \\ \hline
% Vertical HIT &      &  &  & \\ \hline
% Horizontal HIT &      &  &  & \\ \hline
% \end{tabular}
% \end{table}

\paragraph{Encoding range optimization}
We first conduct the parameter selection. As shown in Fig.~\ref{fig:selectiondetail}, our proposed model achieves the best performance at the cut point 8. In case we increase the cut point to 16, the performance of the model is decreasing as more random pixels cannot be learned well. Also, it will slow down and overfit classifiers. Therefore, we adopt the cut point 8 for the rest of our experiments.

==> parts/threatvalidity.tex <==
\paragraph{Adversarial attacks may compromise our approach}
The dataset used for the experiment is quite limited, not only from a malware detection perspective, but also from the DNN training perspective, as typically a quite larger set of dataset required for training DNNs.

Adversarial DL against image classification tasks. It would be more natural to question the robustness of our work in such settings.

About data collection (e.g., are malware and benign drawn from the same timeframe? If not, the classifier may just be learning old from new rather than malicious from benign) and experimental evaluation.

==> structure.tex <==
% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
%\usepackage{epsfig} % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{cite}
\usepackage{algorithmic}
\usepackage{array}
\usepackage{hyperref}
\hypersetup{
    colorlinks = true,
    citecolor=red
}
\usepackage[norelsize]{algorithm2e}
\usepackage[dvipsnames]{xcolor}
\usepackage{subcaption}
